Automated radiotherapy treatment planning guided by GPT-4Vision

Objective: Radiotherapy treatment planning is a time-consuming and potentially subjective process that requires the iterative adjustment of model parameters to balance multiple conflicting objectives. Recent advancements in frontier Artificial Intelligence (AI) models offer promising avenues for addressing the challenges in planning and clinical decision-making. This study introduces GPT-RadPlan, an automated treatment planning framework that integrates radiation oncology knowledge with the reasoning capabilities of large multi-modal models, such as GPT-4Vision (GPT-4V) from OpenAI. Approach: Via in-context learning, we incorporate clinical requirements and a few (3 in our experiments) approved clinical plans with their optimization settings, enabling GPT-4V to acquire treatment planning domain knowledge. The resulting GPT-RadPlan system is integrated into our in-house inverse treatment planning system through an application programming interface (API). For a given patient, GPT-RadPlan acts as both plan evaluator and planner, first assessing dose distributions and dose-volume histograms (DVHs), and then providing textual feedback on how to improve the plan to match the physician's requirements. In this manner, GPT-RadPlan iteratively refines the plan by adjusting planning parameters, such as weights and dose objectives, based on its suggestions. Main results: The efficacy of the automated planning system is showcased across 17 prostate cancer and 13 head and neck cancer VMAT plans with prescribed doses of 70.2 Gy and 72 Gy, respectively, where we compared GPT-RadPlan results to clinical plans produced by human experts. In all cases, GPT-RadPlan either outperformed or matched the clinical plans, demonstrating superior target coverage and reducing organ-at-risk doses by 5 Gy on average (15 percent for prostate and 10-15 percent for head and neck).

==> algorithm.tex <==
\begin{algorithm}[H]
\caption{GPT-RadPlan Auto-Plan Framework}
\label{alg:gpt_radplan}

\textbf{Input:} Patient data ($P$), Reference plans ($R$), Clinical requirements ($C$), Max iterations ($N$) \\
\textbf{Output:} Optimized parameters $w$

\begin{algorithmic}[1]
\State Initialize \textbf{EvaluationModule} with reference cases and clinical objectives
\State Initialize \textbf{MemoryModule} for storing historical trajectories
\State Initialize \textbf{PlanningModule} for generating optimization parameters
\State Extract initial dose distribution $I_0$ and DVH table $\delta_0$ from patient data

\For{$i = 1$ to $N$}
    \State Feedback $F_i \gets \textbf{EvaluationModule}.\text{evaluate}(I_{i-1}, \delta_{i-1})$ \Comment{Evaluate current plan}
    \State \textbf{MemoryModule}.\text{store}($I_{i-1}, \delta_{i-1}, F_i$) \Comment{Store the current state in memory}
    \State $w \gets \textbf{PlanningModule}.\text{plan}(F_i, \textbf{MemoryModule}.\text{getRecentTrajectory}())$
    \Comment{Adjust parameters based on feedback and memory}
    \State $I_i, \delta_i \gets \text{innerLoopOptimization}(w)$ \Comment{Generate new plan using updated parameters}
    \If{$\textbf{EvaluationModule}.\text{isPlanSatisfactory}(I_i, \delta_i)$}
        \State \textbf{break} \Comment{Stop if the plan meets clinical objectives}
    \EndIf
\EndFor
\State \Return $w$
\end{algorithmic}
\end{algorithm}
